Systematic moment expansion for electroweak baryogenesis

We present a systematic moment expansion for solving the semiclassical Boltzmann equations for electroweak baryogenesis. The expansion is developed in powers of adiabatic coordinate velocity, and it is used for computing the CP-violating seed asymmetry at the front of the phase transition wall, that sources the eventual baryon asymmetry of the universe (BAU). We implement the method in a benchmark model, with a CP-violating mass arising from a dimension-5 operator coupling the fermion to a singlet scalar field. We find that the higher moment calculations yield a BAU that can significantly differ from the commonly used two-moment approximation. We discuss in detail the underlying approximations in the moment method and propose a new truncation scheme for the expansion, that appears to give more numerically robust results than the previous schemes.

==> collision-terms.tex <==

\section{Collision terms}

We input the physics of our model into the Boltzmann equation via the collision integral on the right-hand side. For particle species $i$ with distribution $f_i$ and momentum $p_1$, 

\begin{align}
 ( \partial_t + v_z \partial_z + F_z \partial_{p_z} ) f_i = C [f_i] &, \\
 C_{ 2 \to 2} [f_i] = \frac{1}{2 E_1} \int_{p_2, p_3, p_4} | \mathcal{M} |^2 \delta ( p_1 + p_2 - p_3 - p_4) P[ f_i] &; \\
    \int_{p}:= \int {d^3 p}{ ( 2 \pi)^3 2 E}& , \nonumber \\
     P [ f ] = ( f f_2 ( 1 \pm f_3)(1 \pm f_4) - f_3 f_4 ( 1 \pm f ) (1 \pm f_2 ) )&, \\
\end{align}

where - is for fermions (Pauli blocking) and + is for bosons (Bose enhancement). The first, positive contribution to $P [f_i]$ corresponds to particles decaying from state $i$, while the second term corresponds to the production of particle species $i$. The energy is evaluated in the wall frame. %why? 

Similarly, the decay term is 

\begin{align}
  C_{dec} [f_i] = - \frac{1}{2 E_1}  \int_{p_3, p_4} | \mathcal{M} |^2 \delta ( p_1 - p_3 - p_4) P[ f_i] &; \\
  P [ f ] = f ( 1 \pm f_3 ) ( 1 \pm f_4) - f_3 f_4 ( 1 \pm f ) .
\end{align}

We perform a fit to the cross-section functions using the ansatz

\begin{equation} \label{E:cs}
     \sigma_{ij} (s) = \frac{( a + bs + cs^2 )}{v_i s} ,
\end{equation}

where $v_i$ is the velocity of the incoming particle of interest. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Treatment of decay processes}

% define xi
% what's rf?

Using the Maxwell-Boltzmann approximation, the collision term simplifies to

\begin{equation}
    C_{dec} \approx (\xi_3 + \xi_4 - \xi ) f^0_{MB} \frac{|m|}{E_w} \Gamma_{dec}^{rf} - \delta f \frac{|m|}{E_w} \Gamma_{dec}^{rf} + \delta F (p) ,
\end{equation}

where the decay rate is 

\begin{equation}
    \Gamma_{dec}^{rf} = \frac{1}{2 |m|} \int \frac{d^3 p_3}{(2 \pi)^3 2E_3} \frac{d^3 p_4}{(2 \pi)^3 2E_4} (2 \pi)^4 \delta^4 (p - p_3 - p_4) | \mathcal{M}_{dec} |^2
\end{equation}

For a decay cross-section of the form \eqref{E:cs}, we can write

\begin{align}
    [v_{\mol} \sigma] (p_i, p_j) = &\frac{1}{8 p_i p_j E_{p_i} E_{p_j}} \int_{s_-}^{s_+} ds (a + bs + c s^2) \\
             = &\frac{1}{2 E_{p_i} E_{p_j} } \left( a + b (m_i^2 + m_j^2) + c (m_i^2 + m_j^2)^2 \right) + b + 2 (m_i^2 + m_j^2) c \\
             &+ 2 E_{p_i} E_{p_j} c - \frac{p_i^2 p_j^2}{6 E_{p_i} E_{p_j} } c .
\end{align}

%Thus, we encounter a generic integral of the form 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Treatment of inelastic processes}


%CP-even equations, p. 26
For inelastic processes, the collision integral is of the form

\begin{equation}
    C_{inel} \approx (\xi_3 + \xi_4 - \xi_2 - \xi ) f^0_{MB}  \frac{E_p}{E_w} \Gamma_{inel} - \delta f \Gamma_{inel} + \delta F_{inel} (p) ,
\end{equation}

where

\begin{equation}
    \Gamma_{inel} (p) = \frac{1}{2 E_p} \int \frac{d^3 p_2}{(2 \pi)^2 2 E_2 } f_0 (p_2) \flux \sigma_I (s) , 
\end{equation}

and

\begin{equation}
    \flux = 4 E_p E_{p_2} v_{\mol} = 2 \lambda^{1/2} (s, m^2, m_2^2),
\end{equation}

with $\lambda (x, y, z) = (x - y - z)^2 - 4 yz. $


Using the fact that

\begin{equation}
    s = (p + p_2)^2 = 2 m_s^2 + p \cdot p_2 = 2 m_s^2 + 2 E E_2 - 2 p p_2 \cos \theta,
\end{equation}

we can redefine the integration variable and limits 

\begin{align}
    ds = - 2 p p_2 d \cos \theta
    s_\pm = 2 m_s^2 + 2 E E_2 \pm 2 p p_2 = s_0 \pm \Delta s 
\end{align}

and hence 

\begin{equation}
    \int d^3 p_2 = 2 \pi \int dp_2 p_2^2 \frac{1}{2 p p_2 } \int_{s_-}^{s+} ds  = \frac{\pi}{p} \int d p_2 p_2 \int_{s_-}^{s_+} ds .
\end{equation}

Thus

\begin{equation}
    \Gamma_{inel} (p) = d p_2 \frac{p_2^2}{2 \pi^2} [v_{\mol} \sigma_I] (p, p_2) f_0 (E_2) 
\end{equation}

with

\begin{equation}
    [ v_{\mol} \sigma ] (p, p_2) = \frac{1}{8 p_i p_j E_{p_i} E_{p_j}} \int_{s_-}^{s_+} \lambda^{1/2} (s, m^2, m_2^2) \sigma_I (s) .
\end{equation}

%p. 30
For a cross-section of the form \eqref{E:cs}, we can perform the integral numerically. 

We have

\begin{align}
    [v_{\mol} \sigma] = \frac{1}{8 p_i p_j E_{p_i} E_{p_j}} \int_{s_-}^{s^+} ds (a + bs + c s^2)  
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Treatment of elastic processes}

The collision integral for elastic processes takes the form

\begin{align}
    C_{el} \approx - &\frac{1}{E_w} \intp{2} \intp{3} \intp{4} (2 \pi)^4 \delta^4 (p + p_2 - p_3 - p_4 ) \nonumber  \\
      & \cdot | \mathcal{M}_{el} |^2 ( f f_2^{eq} - f_3 f_4^{eq} ) \nonumber \\
     \approx - & \delta f \frac{1}{2 E_w} \intp{2} f_2^{eq} (p) \; \flux \; \sigma_E (s)  + f^{eq} \frac{1}{E_w} \intp{2} \delta f_2 (p_2) \; \flux \; \sigma_E (s) \nonumber \\
     = - &\delta f (p) \frac{E_p}{E_w} \Gamma_{el} + \delta F (p), 
\end{align}

%check distribution function indices above! 

where

%define \Gamma_{el} and \delta F


For a cross-section of the form \eqref{E:cs}, we have




==> discarded-processes.tex <==
\subsubsection{$ t W^- \to b Z$}

The $Wij$ vertex is given by $V^\mu_{Wij} = - i \frac{g_w}{2} \gamma^\mu (1 - \gamma^5) V_{ji}$, where $V_{ij}$ is the element of the CKM matrix corresponding to flavours $i,j$. For the top and bottom quarks, $V_{ji} \approx 1.013.$

The $Zii$ vertex is given by $V^\mu_{Zii} = - i \frac{g_z}{2} \gamma^\mu (v_f - a_f \gamma^5) $.

The couplings are defined by $\cos \theta_w = g/(g^2 + g^\prime^2) = m_W/m_Z$, $g_w = e/\sin \theta_w = 0.646$, $ g_z = e/(\sin \theta_w \cos \theta_w) = 0.735$, $g_{zw} = e \cot \theta_w = 0.568$, $a_f = $, $v_f = $.


\begin{align}
    \Mel_s = &\bar{u}_t (p_3) V^\beta_{Zbb} \frac{\slashed{p_s} + m_b}{p_s^2 - m_b^2} V^\alpha_{Wbt} u_t (p_1) \epsilon_{Z \beta}^{\lambda_4}^\ast (p_4)  \epsilon_{W \alpha}^{\lambda_2} (p_2) \nonumber \\
    \Mel_t = &\bar{u}_t (p_3) V^{\nu}_{Wbt} u_t (p_1) \frac{ ( g^{\nu \delta} - p_t^\nu p_t^\delta / m_W^2)}{p_t^2 - m_W^2) } V_{\delta \alpha \beta} (p_3 - p_2, p_2, -p_4) \epsilon_{Z \beta}^{\lambda_4}^\ast (p_4)  \epsilon_{W \alpha}^{\lambda_2} (p_2) \nonumber \\
    \Mel_u =  &\bar{u}_t (p_3) V^\alpha_{Wbt} \frac{\slashed{p_u} + m_t}{p_u^2 - m_t^2} V^\beta_{Zbb}  u_t (p_1) \epsilon_{Z \beta}^{\lambda_4}^\ast (p_4)  \epsilon_{W \alpha}^{\lambda_2} (p_2) . 
\end{align}


\subsubsection{$ H Z \to W^+ W^-$}

\begin{align}
    \Mel_s = & (  g_{zw} g_z m_Z ) \frac{( g^{\nu \delta} - p_s^\nu p_s^\delta / m_Z^2)}{q^2 - m_z^2) } V_{\delta \alpha \beta} (p_s,-p_3,-p_4) \epsilon_\nu^{\lambda_2} (p_2) \epsilon_\alpha^{\lambda_3}^\ast (p_3) \epsilon_\beta^{\lambda_4}^\ast (p_4) \nonumber \\
     \Mel_t =& ( g_{zw} g_w m_W  V_{\mu \beta \nu} (p_2, -p_4, p_4 - p_2  ) \frac{ ( g^{\nu \delta} - p_t^\nu p_t^\delta / m_W^2)}{p_t^2 - m_W^2) } \epsilon_\mu^{\lambda_2} (p_2) \epsilon_{\delta}^{\lambda_3}^\ast (p_3) \epsilon_\beta^{\lambda_4}^\ast (p_4) \nonumber \\
     \Mel_u = & \Mel_t (p_3 \leftrightarrow p_4 ). 
\end{align}


\subsubsection{$ H W \to Z W $}

\begin{align}
    \Mel_s = & g_{zw} g_w g_{\mu \alpha} \frac{ ( g^{\alpha \delta} - p_s^\alpha p_s^\delta / m_W^2)}{p_s^2 - m_w^2) } V_{\delta \gamma \nu} (q,-p_3,-p_4) \epsilon_\mu^{\lambda_2} (p_2) \epsilon_\gamma^{\lambda_3}^\ast (p_3) \epsilon_\nu^{\lambda_4}^\ast (p_4)  \nonumber \\
    \Mel_t = & g_{zw} g_z g_{\alpha \gamma} \frac{( g^{\alpha \delta} - p_t^\alpha p_t^\delta / m_Z^2)}{p_t^2 - m_Z^2} V_{\delta \mu \nu} ( p_3 - p_2, p_2, -p_4) 
    \epsilon_\mu^{\lambda_2} (p_2) \epsilon_\gamma^{\lambda_3}^\ast (p_3) \epsilon_\nu^{\lambda_4}^\ast (p_4) \nonumber \\
     \Mel_u = & \Mel_t (p_3 \leftrightarrow p_4 ). 
\end{align}


==> generic-integrals.tex <==
\section{Integrals}

We encounter generic integrals of the form

\begin{align}
\frac{1}{2 \pi^2 } \int dp_j p_j^{2n} E_j^{\alpha} f^{eq} (p_j) 
= \int dE_j 

\end{align}

==> list-of-processes.tex <==
$Q$ refers to up, down, charm and strange quarks; we neglect their masses and sum over them with a front factor $N_f = 4$.

\subsection{Helicity-violating processes: helicity flip}


\subsubsection{$t_L$, $t_R$ processes}


Since the cross-sections only depend on the product of the helicities, $ t_L \to t_R$ and $ t_R \to t_L$ have the same cross-section. Processes with distinct cross-sections are listed in bold; the others are simply duplicates of the others, as indicated. 

The cross-sections in our code correspond to one helicity combination, either $ t_R \to t_L$ or $t_L \to t_R$ (that is to say, we include helicity projectors substitute $ \lambda_1 \lambda_3 = 1$). However, when two distinct processes have the identical cross-section (for example, when $Q$ is replaced by $\bar{Q}$) we sum these two processes together as one cross-section for a specific helicity combination. 

\begin{enumerate}
 \item $t_L H \to t_R g$ , $t_R H \to t_L g$ 
 \item $t_L g \to t_R H$ , $t_R g \to t_L H$ 
 \item $t_L Q \to t_R Q$ , $t_R Q \to t_L Q$ 
 \item $t_L \bar{Q} \to t_R \bar{Q}$ , $t_R \bar{Q} \to t_L \bar{Q}$ 
 \item $ t_L b \to t_R b$ , $ t_R b \to t_L b$ 
 \item $ t_L \bar{b} \to t_R \bar{b}$ , $ t_R \bar{b} \to t_L \bar{b}$ 
 \item $t_L t \to t_R t$ ,  $t_R t \to t_L t$ 
 \item $t_L \bar{t} \to t_R \bar{t}$ ,  $t_R \bar{t} \to t_L \bar{t}$ 
 \item $t_L g \to t_R g$ , $t_R g \to t_L g$ 
 \end{enumerate}
 
 
 \subsubsection{$b_L$ processes}
 
Processes in bold have been calculated separately, since they depend on both $m_t$ and $m_b$; the others are simply the same processes as above, with $m_t$ replaced by $m_b$. 
 
 \begin{enumerate}
  \item $b_L H \to b_R g$ 
  \item $b_L g \to b_R H$ 
  \item $b_L Q \to b_R Q$ 
  \item $b_L t \to b_R t $
  \item $b_L \bar{Q} \to b_R \bar{Q}$ 
  \item $b_L \bar{t} \to b_R \bar{t}$
  \item $b_L b \to b_R b$  
  \item $b_L \bar{b} \to b_R \bar{b}$ 
  \item $b_L g \to b_R g$ 
 \end{enumerate}
 

\subsection{Helicity-violating processes: Annihilation processes}

We calculate the helicity-violating cross-sections for these processes (we use the convention that $\Prj{i} (p_i) = ( 1 + \lambda_i \g^5 \slashed{s_i})/2 $ for both particles and antiparticles, and choose the processes for which $\lambda_1 \lambda_2 = 1$). As before, the processes that needed to be calculated separately are boldfaced. 

\subsubsection{$t_L$, $t_R$ processes}
\begin{enumerate}
 \item $t \bar{t} \to gg$ 
 \item $t \bar{t} \to Q \bar{Q}$ 
 \item $t \bar{t} \to b \bar{b}$ 
 \item $t \bar{t} \to t \bar{t}$ 
\end{enumerate}

\subsubsection{$b_L$ processes}
\begin{enumerate}
 \item $b \bar{b} \to gg$
 \item $b \bar{b} \to Q \bar{Q}$
 \item $b \bar{b} \to t \bar{t} $ 
 \item $b \bar{b} \to b \bar{b}$ 
\end{enumerate}


\subsection{Elastic processes}

For the CP-even collision integral, we compute the unpolarised cross-sections, averaging over the two helicity states of the incoming top quark (we sum over the helicity states of the other incoming particle and the outgoing particles).


\subsubsection{$t$ processes}


\begin{enumerate}
  \item $ t Q \to t Q$ 
  \item $t \bar{Q} \to t \bar{Q}$ (same cross-section) 
  \item $ t g \to t g$ 
  \item $t t \to t t $ 
  \item $ t \bar{t} \to t \bar{t}$ 
\end{enumerate}

\subsubsection{$b_L$ processes}

\begin{enumerate}
  \item $ b Q \to b Q$ 
  \item $ b \bar{Q} \to b \bar{Q}$ (same cross-section) 
  \item $ b g \to b g$ 
  \item $ b t \to b t $ 
  \item $ b \bar{t} \to b \bar{t}$ 
\end{enumerate}

\subsubsection{$t-b_L$ processes}

\begin{enumerate}
\item $ t b \to t b$ 
\item $ t \bar{b} \to t \bar{b} $ (same cross-section) 
\end{enumerate}



\subsection{Gauge boson $2 \to 2$ processes}

\begin{enumerate}
  \item $H Z \to W^+ W^-$ , $ H W^+ \to Z W^+$, $ H W^- \to Z W^-$
  \item $ t W^- \to b Z$ 
\end{enumerate}


==> matrix-elements-old.tex <==
\section{Matrix elements}
%note on symmetry factors

\subsection{Yukawa processes}

The Lagrangian giving rise to Yukawa processes is
%
\begin{equation}
\mathcal{L} = -y_t\big( \bar{Q}_{\rm L}\tilde Ht_{\rm R} + \bar{t}_{\rm R}\tilde H^\dagger Q_{\rm L} \big)  +  g_s \bar q_i \slashed A^at^a_{ij}q_j.
\end{equation}
%
where $Q_L \equiv (t_{\rm L},b_{\rm L})^T$ and $\tilde H \equiv i\sigma_2H^* = (h^*,-h^-)^T$. The processes created by these interactions include channels $g t_{\lambda} \to \tilde H^*  Q_{\lambda'}$,$\tilde H t_{\lambda} \to g Q_{\lambda'}$ and $t_\lambda Q^c_{\lambda'} \to g \tilde H^*$. The matrix elements for these processes are given by
%
\begin{align}
    \Mel_{g t_{\lambda} \to \tilde H^* Q_{\lambda'}} =& iy_tg_s \bar{u}_Q^{\lambda'} (p_4) \Big[ P_R \frac{1}{\slashed{p}_s \!-\! m_t }\slashed{\epsilon}_2  + \slashed{\epsilon}_2 \frac{1}{\slashed{p}_t \!-\! m_Q} P_R  \Big] u_t^{\lambda} (p_1),
    \\
    \Mel_{\tilde H t_{\lambda} \to g Q_{\lambda'}} =& iy_tg_s \bar{u}_Q^{\lambda'} (p_3) \Big[ P_R \frac{1}{\slashed{p}_u \!-\! m_t} \slashed{\epsilon}_4 +\slashed{\epsilon}_4 \frac{1}{\slashed{p}_s \!-\! m_Q }P_R  \Big] u_t^{\lambda} (p_1),
    \\ 
    \Mel_{t_{\lambda} Q^c_{\lambda'} \to g \tilde H^*} =& iy_tg_s \bar{v}_Q^{\lambda'} (p_2) \Big[ P_R \frac{1}{\slashed{p}_t \!-\! m_t } \slashed{\epsilon}_3  + \slashed{\epsilon}_3 \frac{1}{\slashed{p}_u \!-\! m_Q} P_R  \Big] u_t^{\lambda} (p_1),
\end{align}
%
where $\slashed{\epsilon}_i \equiv \gamma^\mu\epsilon_\mu^a(p_i)t^a$ and $p_s = p_1+p_2$, $p_t = p_1-p_3$ and $p_u = p_1-p_4$ and we suppressed the obvious SU(3)-indexing in spinors and the generator $t^a$. The processes involving antiparticles have identical rates with the particle channels with  opposite helicities: 
%
\begin{align}
\Gamma(g t^c_{\lambda} \to \tilde H Q^c_{\lambda'}) \;=& \;\; \Gamma(g t_{-\lambda} \to \tilde H^* Q_{-\lambda'})
\nonumber \\
\Gamma(\tilde H^* t^c_{\lambda} \to g Q^c_{\lambda'}) \;=& \;\;\Gamma(\tilde H t_{-\lambda} \to g Q_{-\lambda'}) 
\nonumber \\
\Gamma(t^c_{\lambda}Q_{\lambda'} \to g\tilde H) \;=& \;\; \Gamma(t_{-\lambda} Q^c_{-\lambda'} \to g \tilde H^*).
\label{eq:complex-identitites}
\end{align}
%
This means that antiparticles contribute to the CP-odd collision integrals exactly the same way as particles, so that the rates appearing in the CP-odd collision integrals in the CP-odd perturbation equation~\cref{eq:bolzmann_equationdel2} computing just particle sector coefficients. Of course, in all cases the inverse process has the same rate as the direct process by the detailed balance:
%
\begin{equation}
\Gamma(ab \to cd) =& \Gamma(cd \to ab). 
\label{eq:detailed-balance}
\end{equation}
%
This implies that 
$\Gamma(\tilde H^* Q_{\lambda} \to g t_{\lambda'})=\Gamma(g t_{\lambda'} \to \tilde H^* Q_{\lambda})$ and $\Gamma(g Q_{\lambda} \to \tilde H t_{\lambda'})=\Gamma(\tilde H t_{\lambda'} \to g Q_{\lambda})$. In addition there is an open decay channel created by the Yukawa interaction: $t_\pm \rightarrow b_- h^+$. The decay width is easy to compute: $\Gamma_{t_\pm \rightarrow b_- h^+} = y_t^2m_t/(32\pi)$. We can now write down the rate terms coming from Yukawa-interactions in the equation for $\tR$ for example:
%
\begin{align}
{\bar C}_{\tR} &= \big[\Gamma_{g\tR\rightarrow h\tL} + \Gamma_{h^*\tR\rightarrow g\tL} +                                   \Gamma_{\tR t^c_- \rightarrow g h}\big] (\mu_\tR \!-\! \mu_\tL \!-\! \mu_h)
\nonumber\\ 
               &+ \big[\Gamma_{g\tR\rightarrow h^+\bL} + \Gamma_{h^-\tR\rightarrow g\bL} + 
                  \Gamma_{\tR b^c_- \rightarrow g h^+}+\Gamma_{t_\pm \rightarrow b_- h^+} \big] 
                  (\mu_\tR \!-\! \mu_\bL \!-\! \mu_{h^+})
\nonumber\\ 
               &+ \big[\Gamma_{g\tL\rightarrow h\tR} + \Gamma_{h^*\tL\rightarrow g\tR} + 
                  \Gamma_{\tL t^c_+ \rightarrow g h} \big] (\mu_\tR \!-\! \mu_\tL \!+ \!\mu_{h})
\nonumber\\
               &- \big[ \Gamma_{\tR t^c_+ \rightarrow g h}
                     - \Gamma_{\tL t^c_- \rightarrow g h} \big] \mu_{h}.
\end{align}
%
%            - &\;\; \big[ \Gamma_{g\tR\rightarrow h\tR} + \Gamma_{h^*\tR\rightarrow g\tR} + 
%                         \Gamma_{\tR t^c_+ \rightarrow g h}
%            - \Gamma_{g\tR\rightarrow h\tR} - \Gamma_{h\tR\rightarrow g\tR} - 
%                         \Gamma_{\tL t^c_- \rightarrow g h} \big] \mu_{h}
%
Here the terms on third line and last term in the fourth line correspond to processes where $\tL$ comes from an isospin doublet in the initial state. The third-line terms were then rewritten using the detailed balance condition~\cref{eq:detailed-balance} and the last term in fourth line using~\cref{eq:complex-identitites}. After a little further rearranging, we can write $\bar C_\tR$ in the form appearing in equation~\cref{eq:collision_terms2a}:
%
\begin{equation}
{\bar C}^{y_tg_s}_\tR = \tsum_\pm \Gamma^t_\pm (\mu_\tR \!\!-\! \mu_\tL \!\!\mp\! \mu_h )
                      + \Gamma^b_+ (\mu_\tR \!\!-\! \mu_\bL \!\!-\! \mu_{h^+}) 
                      - \Gamma_{ht} \mu_h ,
\end{equation}
% 
where $\tGamma^t \equiv \sum_\pm \tGamma^t_{\sss \pm}$ and
%
\begin{align}
\Gamma^t_\pm  &= \Gamma_{gt_\pm\rightarrow ht_\mp} 
               + \Gamma_{h^*t_\pm \rightarrow gt_\mp}
               + \Gamma_{t_\pm t^c_\mp \rightarrow g h} 
\nonumber \\
\Gamma^b_\pm  &= \Gamma_{gt_\pm \rightarrow h^+\bL} 
               + \Gamma_{h^-t_\pm \rightarrow g\bL}  
               + \Gamma_{t_\pm b^c_- \rightarrow g h^+} 
               + \Gamma_{t_\pm \rightarrow b_- h^+}
\nonumber \\
\Gamma^{ht}   &= \Gamma_{t_+ t^c_+ \rightarrow g h} - \Gamma_{t_- t_-^c \rightarrow g h} 
\end{align}
%
In the massless limit only the rates $\Gamma_{g\tR \rightarrow h\tL}$ and $\Gamma_{g\tR \rightarrow h\bL}$ are nonzero and reproduce the terms included in~\cite{Cline:2020jre}. Similarly, one can write  the collision integrals for $\tL$, $\bL$, $h$ and $h^+$ in rather simple forms as follows:
%
\begin{align}
{\bar C}^{y_tg_s}_\tL &= \tsum_\pm \Gamma^t_\pm (\mu_\tL \! - \! \mu_\tR \! \pm \! \mu_h )
                                  + \Gamma^b_-  (\mu_\tL \! - \! \mu_\bL \! +   \! \mu_{h^+}) 
                                  + \Gamma^{ht} \mu_h ,
\nonumber \\
{\bar C}^{y_tg_s}_\bL &= \tsum_\pm \Gamma^b_\pm  (\mu_\bL \! - \! \mu_{t_\pm} \! - \! \mu_{h^+} )
\nonumber \\
{\bar C}^{y_tg_s}_h     &= \tsum_\pm \Gamma^t_\pm  (\mu_h \! + \! \mu_{t_\pm} \! - \! \mu_{t_\mp} ) + \Gamma^h_{\sss W} \mu_h
\nonumber \\
{\bar C}^{y_tg_s}_{h^+} &= \tsum_\pm \Gamma^b_\pm  (\mu_h \! + \! \mu_{t_\pm} \! - \! \mu_{b_-} ) -  
\Gamma^h_{\sss W} \mu_{h^+},
\end{align}
%
where finally 
%
\begin{equation}
\Gamma^h_\pm  = \Gamma_{t_\pm t^c_\mp \rightarrow g h} - \Gamma_{t_\mp t_\mp^c \rightarrow g h} 
\end{equation}
%
Again, in the chiral limit $\Gamma^{t,b}_- \rightarrow 0$ and ...

\begin{align}
    i \Mel_s &= \bar{u}_t^{\lambda_3} (p_3)_j (i g_s \gamma^\mu t^a_{ji} ) \frac{ \slashed{p}_1 + \slashed{p}_2 + m_t }{s - mt^2} \frac{y_t}{\sqrt{2}} u_t^{\lambda_1} (p_1) \epsilon^\ast_\mu (p_4 )    \\
   i \Mel_u &= \bar{u}_t^{\lambda_3} (p_3) \frac{y_t}{\sqrt{2}} \frac{ \slashed{p}_1 - \slashed{p}_4 + m_t }{u - mt^2} (i g_s \gamma^\mu t^a_{ji} ) u_t^{\lambda_1} (p_1) \epsilon^\ast_\mu (p_4 ).  \\
\end{align}
%
\subsubsection{$ Q t_L \to Q t_R $ }

We define
%
\begin{equation}
  V_{\alpha\beta\gamma}(p_1,p_2,p_3) := g_{\alpha \beta} (p_1 - p_2)_\gamma + g_{\beta \gamma} (p_2 - p_3)_\alpha + g_{\gamma \alpha} (p_3 - p_1)_\beta .
\end{equation}
%
Processes with identical cross-sections are summed together (for example, $ t Q \to t Q$ and $ t \bar{Q} \to t \bar{Q}$ ). 

\begin{equation}
     \Mel_t = \frac{ g_s^2}{t - M_g^2} t^a_{ij} t^a_{kl} \bar{u}_t^{\lambda_3} (p_3)  \gamma^\mu    u_t^{\lambda_1} (p_1)  \;\; \bar{u}_Q (p_4)  \gamma_\mu   u_Q (p_2) .
\end{equation}

\subsubsection{$ \bar{Q} t_L \to \bar{Q} t_R $ }

\begin{equation}
    \Mel_t = \frac{ g_s^2}{t - M_g^2} t^a_{ij} t^a_{kl} \bar{u}_t^{\lambda_3} (p_3) \gamma^\mu  u_t^{\lambda_1} (p_1) \;\;  \bar{v}_Q (p_2) \gamma_\nu v_Q (p_4) .
\end{equation}

\subsubsection{ $ t_L t \to t_R t $ }

\begin{align}
 \mathcal{M}_t = \frac{ g_s^2}{t - M_g^2} t^a_{ji} t^a_{lk} \bar{u}_t^{\lambda_3} (p_3)  \gamma^\mu    u_t^{\lambda_1} (p_1) \;\; \bar{u}_t (p_4)  \gamma_\mu   u_t (p_2) \nonumber \\
  \mathcal{M}_u = \frac{ g_s^2}{u - M_g^2} t^a_{li} t^b_{jk} \bar{u}_t (p_4)  \gamma^\mu  u_t^{\lambda_1} (p_1)  \;\; \bar{u}_t^{\lambda_3} (p_3) \gamma_\mu u_t (p_2) .
\end{align}

\subsubsection{ $ t_L \bar{t} \to t_R \bar{t} $ }

\begin{align}
    \Mel_s &= \frac{ g_s^2}{s} t^a_{ij} t^a_{lk} \bar{v}_t (p_2)  \gamma^\mu   u_t^{\lambda_1} (p_1)  \;\; \bar{u}_t^{\lambda_3} (p_3)  \gamma_\mu   v_t (p_4) \nonumber \\
    %%%%%%%
    \Mel_t &= \frac{ g_s^2}{t - M_g^2} t^a_{ik} t^a_{lj} \bar{u}_t^{\lambda_3} (p_3)  \gamma^\mu   u_t^{\lambda_1} (p_1) \;\; \bar{v}_t (p_2) \gamma_\mu   v_t (p_4). 
\end{align}


\subsubsection{ $g t_L \to g t_R $ }
%note on gauge

\begin{align}
   \mathcal{M}_s = & - g_s^2 \bar{u}_t^{\lambda_3} (p_3) \slashed{\epsilon}_4^\ast \frac{ (\slashed{p}_1 + \slashed{p}_2 + m_t)}{s - m_t^2} \slashed{\epsilon}_2  u_t^{\lambda_1} (p_1) \nonumber \\
  %%%%%
  \mathcal{M}_t = & \frac{i g_s^2}{t - M_g^2} t^c_{ki} f^{cad} \bar{u}_t^{\lambda_3} (p_3) (i \gamma^\mu   ) u_t^{\lambda_1} (p_1)  \epsilon^\ast_\beta ( p_4) \epsilon_\alpha (p_2) \nonumber \\
  & \cdot  V_{\mu \alpha \beta} (p_1 -p_3, p_2, -p_4) \nonumber \\
  %%%%%
  \mathcal{M}_u = & i g_s^2 \bar{u}_t^{\lambda_3} (p_3) \slashed{\epsilon}_2  \frac{i (\slashed{p}_1 - \slashed{p}_4 + m_t)}{ u - m_t^2} \slashed{\epsilon}_4^\ast u_t^{\lambda_1} (p_1) .
\end{align}

\subsection{ $ t \bar{t} \to Q \bar{Q} $}

%check
\begin{equation}
   %\sigma = \frac{2 m_t^2+s}{6 \pi  \sqrt{s^3 \left(s-4 m_t^2\right)}} .
   \mathcal{M}_ s = \frac{g_s^2}{s} t^a_{ji} t^a_{kl} \bar{v_t}^{\lambda_2} (p_2)  ( \gamma^\mu  ) u_t^{\lambda_1} (p_1) \bar{u}_Q (p_3) (\gamma_\mu  ) v_Q (p_4).
\end{equation}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Elastic processes}

\subsubsection{ $ g t \to g t $ }


\subsubsection{ $ t Q (\bar{Q}) \to t Q (\bar{Q}) $} 
\subsubsection{ $ t t \to t t $}

\subsubsection{ $ t \bar{t} \to t \bar{t} $}


\subsection{Annihilation processes}



\subsection{ $ t \bar{t} \to t \bar{t} $ }

\begin{align}
 \mathcal{M}_ s = \frac{g_s^2}{s} t^a_{ji} t^a_{kl} \bar{v_t}^{\lambda_2} (p_2)  \gamma^\mu   u_t^{\lambda_1} (p_1) \;\; \bar{u}_t (p_3)  \gamma_\mu   v_t (p_4) \nonumber \\
 %%%%%%
 \mathcal{M}_t = \frac{g_s^2}{t - M_g^2} t^a_{ki} t^a_{jl} \bar{u}_t (p_3)  \gamma^\mu  u_t^{\lambda_1} (p_1) \;\; \bar{v}_t^{\lambda_2} (p_2)  \gamma_\mu    v_t (p_4) .
\end{align}


\subsubsection{ $ t \bar{t} \to g g $ }

\begin{align}
  \mathcal{M}_s = & \frac{- i g_s^2}{s} t^a_{ij} f^{acd} \bar{v}_t^{\lambda_2} (p_2)   \gamma^\mu   u_t^{\lambda_1} (p_1)     V_{\mu \alpha \beta} (p_1 + p_2, -p_3, -p_4 ) \epsilon^\ast_\alpha (p_3) \epsilon^\ast_\beta (p_4) \nonumber \\
 %%%%%
  \mathcal{M}_t = & g_s^2  \bar{v}_t^{\lambda_2} (p_2)    \slashed{\epsilon}^\ast_4   \frac{ ( \slashed{p}_1 - \slashed{p}_3 + m_t)}{ t - m_t^2} \slashed{\epsilon}_3   u_t^{\lambda_1} (p_1) \nonumber \\
 %%%%%% 
 \mathcal{M}_u = & g_s^2 \bar{v}_t^{\lambda_2} (p_2)    \slashed{\epsilon}_3  \frac{ i ( \slashed{p}_1 - \slashed{p}_4 + m_t)}{ u - m_t^2}  \slashed{\epsilon}_4^\ast u_t^{\lambda_1} (p_1) .
\end{align}


\subsection{Vector boson processes}

\subsubsection{$ t W^- \to b Z$}


\subsubsection{$ H Z \to W^+ W^-$}

\begin{align}
    \Mel_s = & (  g_{zw} g_z m_Z ) \frac{( g^{\nu \delta} - q^\nu q^\delta / m_Z^2}{q^2 - m_z^2) } V_{\delta \alpha \beta} (q,-p_3,-p_4) \epsilon_\nu^{\lambda_2} (p_2) \epsilon_\alpha^{\lambda_3}^\ast (p_3) \epsilon_\beta^{\lambda_4}^\ast (p_4), \nonumber \\
    & q = p_1 + p_2 . \nonumber \\
     \Mel_t =& ( g_{zw} g_w m_W  V_{\mu \beta \nu} (p_2, -p_4, p_4 - p_2  ) \frac{ ( g^{\nu \delta} - q^\nu q^\delta / m_W^2}{q^2 - m_W^2) } \epsilon_\mu^{\lambda_2} (p_2) \epsilon_{\delta}^{\lambda_3}^\ast (p_3) \epsilon_\beta^{\lambda_4}^\ast (p_4), \nonumber \\
    & q = p_1 - p_3 . \nonumber \\
     \Mel_u = & \Mel_t (p_3 \leftrightarrow p_4 ). 
\end{align}


\subsubsection{$ H W \to Z W $}

\begin{align}
    \Mel_s = & g_{zw} g_w g_{\mu \alpha} \frac{ ( g^{\alpha \delta} - q^\alpha q^\delta / m_W^2}{q^2 - m_w^2) } V_{\delta \gamma \nu} (q,-p_3,-p_4) \epsilon_\mu^{\lambda_2} (p_2) \epsilon_\gamma^{\lambda_3}^\ast (p_3) \epsilon_\nu^{\lambda_4}^\ast (p_4) ,
    \nonumber \\
     & q = p_1 + p_2 . \nonumber \\
    \Mel_t = & g_{zw} g_z 
\end{align}

